Efficient Methods for Unsupervised Learning of Probabilistic Models

In this thesis I develop a variety of techniques to train, evaluate, and sample from intractable and high dimensional probabilistic models. Abstract exceeds arXiv space limitations -- see PDF.

==> Makefile <==
# THESIS-IN-A-BOX Makefile

# Paths to the programs used by this Makefile.
PDFLATEX = pdflatex
BIBTEX = bibtex
MAKEINDEX = makeindex
CP = cp
RM = rm
GREP = grep
DIFF = diff -q
TOUCH = touch

# Paths to the input and output files.  These can be changed.
TEXFILE = thesis.tex 
BIBFILE = thesis.bib
PDFFILE = thesis.pdf
TEXINCLUDES = dedication.tex abstract.tex \
              frontmatter.sty acknowledgements.tex commands.tex \
              hyperref.cfg thesis.tex frontmatter.tex \
              commands.tex \
              chap_mpf.tex chap_mpf_examples.tex chap_hais.tex chap_intro.tex chap_conclusion.tex chap_HMC.tex chap_natgrad.tex chap_natgrad_body.tex chap_conclusion.tex \
	      app_MPF_taylor.tex app_MPF_ising.tex app_MPF_RBM.tex app_SM_MPF.tex app_MPF_convex.tex  app_MPF_bound.tex              

# Paths to intermediate files that are created by the make process.
# Do not change these.
TEXLOG = $(basename $(TEXFILE)).log
BIBLIOGRAPHYFILE = $(basename $(TEXFILE)).bbl
BIBTEXLOG = $(basename $(TEXFILE)).blg
INDEXFILE = $(basename $(TEXFILE)).ind
MAKEINDEXLOG = $(basename $(TEXFILE)).ilg
AUXFILE = $(basename $(TEXFILE)).aux
OLDAUXFILE = ".$(AUXFILE).old"
TOCFILE = $(basename $(TEXFILE)).toc
OUTFILE = $(basename $(TEXFILE)).out
INDEXITEMFILE = $(basename $(TEXFILE)).idx
OLDINDEXITEMFILE = ".$(INDEXITEMFILE).old"

# If this message appears in TEXLOG, we must re-run LaTeX.
RERUNLATEX = "Rerun to get cross-references right"

# The primary target (created by the command "make") is the PDF file.
pdf: $(PDFFILE)

# This rule uses PDFLaTeX to create a PDF file from a LaTeX file.  If
# the AUX file has changed, then the BIB file is updated.  If the IDX
# file has changed then the IND file is updated. Then the PDFLaTeX is
# re-run to resolve references, as necessary.
$(PDFFILE): $(TEXFILE) $(TEXINCLUDES) $(BIBFILE) 
	$(TOUCH) $(AUXFILE)
	$(TOUCH) $(INDEXITEMFILE)
	$(CP) $(AUXFILE) $(OLDAUXFILE)
	$(CP) $(INDEXITEMFILE) $(OLDINDEXITEMFILE)
	$(PDFLATEX) $<
	if ! $(DIFF) $(AUXFILE) $(OLDAUXFILE); then $(BIBTEX) $(basename $<); $(PDFLATEX) $<; fi
	if ! $(DIFF) $(INDEXITEMFILE) $(OLDINDEXITEMFILE); then $(MAKEINDEX) $(INDEXITEMFILE); $(PDFLATEX) $<; fi
	while $(GREP) -q $(RERUNLATEX) $(TEXLOG); do $(PDFLATEX) $<; done

# This rule cleans out the files made by the make process.
clean:
	$(RM) -f $(AUXFILE) \
                 $(OLDAUXFILE) \
                 $(TEXLOG) \
                 $(TOCFILE) \
                 $(OUTFILE) \
                 $(BIBLIOGRAPHYFILE) \
                 $(BIBTEXLOG) \
                 $(INDEXFILE) \
                 $(INDEXITEMFILE) \
                 $(OLDINDEXITEMFILE) \
                 $(MAKEINDEXLOG) \
                 $(PDFFILE)



==> Makefile_ <==
# THESIS-IN-A-BOX Makefile

# Paths to the programs used by this Makefile.
PDFLATEX = pdflatex
BIBTEX = bibtex
MAKEINDEX = makeindex
CP = cp
RM = rm
GREP = grep
DIFF = diff -q
TOUCH = touch

# Paths to the input and output files.  These can be changed.
TEXFILE = thesis.tex 
BIBFILE = thesis.bib
PDFFILE = thesis.pdf
TEXINCLUDES = dedication.tex abstract.tex \
              frontmatter.sty acknowledgements.tex commands.tex \
              hyperref.cfg thesis.tex frontmatter.tex \
              commands.tex \
              chap_mpf.tex chap_mpf_examples.tex chap_hais.tex chap_intro.tex chap_conclusion.tex chap_HMC.tex chap_natgrad.tex chap_natgrad_body.tex \
	      app_MPF_taylor.tex app_MPF_ising.tex app_MPF_RBM.tex app_SM_MPF.tex app_MPF_convex.tex  app_MPF_bound.tex              

# Paths to intermediate files that are created by the make process.
# Do not change these.
TEXLOG = $(basename $(TEXFILE)).log
BIBLIOGRAPHYFILE = $(basename $(TEXFILE)).bbl
BIBTEXLOG = $(basename $(TEXFILE)).blg
INDEXFILE = $(basename $(TEXFILE)).ind
MAKEINDEXLOG = $(basename $(TEXFILE)).ilg
AUXFILE = $(basename $(TEXFILE)).aux
OLDAUXFILE = ".$(AUXFILE).old"
TOCFILE = $(basename $(TEXFILE)).toc
OUTFILE = $(basename $(TEXFILE)).out
INDEXITEMFILE = $(basename $(TEXFILE)).idx
OLDINDEXITEMFILE = ".$(INDEXITEMFILE).old"

# If this message appears in TEXLOG, we must re-run LaTeX.
RERUNLATEX = "Rerun to get cross-references right"

# The primary target (created by the command "make") is the PDF file.
pdf: $(PDFFILE)

# This rule uses PDFLaTeX to create a PDF file from a LaTeX file.  If
# the AUX file has changed, then the BIB file is updated.  If the IDX
# file has changed then the IND file is updated. Then the PDFLaTeX is
# re-run to resolve references, as necessary.
$(PDFFILE): $(TEXFILE) $(TEXINCLUDES) $(BIBFILE) 
	$(TOUCH) $(AUXFILE)
	$(TOUCH) $(INDEXITEMFILE)
	$(CP) $(AUXFILE) $(OLDAUXFILE)
	$(CP) $(INDEXITEMFILE) $(OLDINDEXITEMFILE)
	$(PDFLATEX) $<
	if ! $(DIFF) $(AUXFILE) $(OLDAUXFILE); then $(BIBTEX) $(basename $<); $(PDFLATEX) $<; fi
	if ! $(DIFF) $(INDEXITEMFILE) $(OLDINDEXITEMFILE); then $(MAKEINDEX) $(INDEXITEMFILE); $(PDFLATEX) $<; fi
	while $(GREP) -q $(RERUNLATEX) $(TEXLOG); do $(PDFLATEX) $<; done

# This rule cleans out the files made by the make process.
clean:
	$(RM) -f $(AUXFILE) \
                 $(OLDAUXFILE) \
                 $(TEXLOG) \
                 $(TOCFILE) \
                 $(OUTFILE) \
                 $(BIBLIOGRAPHYFILE) \
                 $(BIBTEXLOG) \
                 $(INDEXFILE) \
                 $(INDEXITEMFILE) \
                 $(OLDINDEXITEMFILE) \
                 $(MAKEINDEXLOG) \
                 $(PDFFILE)



==> clippings.tex <==













%A range of spatial and temporal representations may be obtained by applying
%the model hierarchically to its own output.

%Recent advances in computer vision have bestowed machines with a limited
%ability to process and derive meaningful conclusions from visual input, but
%there remains a wide gulf between the abilities of these machines and those of
%biological systems that see.  Following the work of
%Attneave~\cite{attneave54}, Barlow~\cite{barlow61}, Atick and
%Redlich~\cite{atick92}, Olshausen and Field~\cite{olshausen96emergence},
%Bell and Sejnowski~\cite{bell97}, and many others~\cite{Wallis97,
%wiskott02slowfeature, einhauser02learning,hyvarinen03bubbles}, the goal of
%this research is a statistical model of natural scenes.
%We hope that by understanding the algorithms used by the biological system
%we can inform and accelerate algorithm development in machine vision,
%and eventually endow machines with abilities on par with their
%biological counterparts.  The goal of this paper is the formulation
%and evaluation of a model that demonstrates functionality similar to the
%ability of cortex to separate sensory information coming into the eye into
%two streams along two distinct pathways: ventral (`what') and dorsal
%(`where' or `how'). We believe that the benefit this function provides
%to biological vision systems can be transferred to machine vision algorithms.
%
%Strong support for this idea of two streams comes from lesion studies in   
%monkeys, in which damage to dorsal or ventral cortical regions impairs
%abilities of spatial perception or object identification,
%respectively~\cite{ungerleider82, milner95}.  Little is known about the
%methods by which cortex obtains these separate representations,
%but there are suggestions that the methods are applied hierarchically:
%there is anatomical evidence for additional function streams, or `streams
%within streams'~\cite{deyoe94}.  This paper investigates the feasibility of
%accomplishing this separation by combining two powerful principles for
%pattern recognition with bilinear generative models.  The method described
%herein is consistent with some physiological evidence and can be applied
%hierarchically to its own output to obtain a range of temporal and spatial
%representations.

%In section 2, we begin by reviewing \emph{sparse coding} -- the main
%machinery we utilize for learning -- as an E-M algorithm, then examine it in
%the context of a linear generative model for `what' in natural images.
%Section 3 describes two linear generative models and E-M algorithms for
%learning `where' from natural movies.  Section 4 shows how these ideas merge
%naturally together into a bilinear generative model for natural movies that
%makes the separation between `what' and `where' explicit.
%In section 5 we conclude.














%, and after running
%another E-M algorithm we show that this model is capable of coding test
%videos using less bits than the other models.  

%\begin{table}[t]
%\caption{Sample table title}
%\label{sample-table}
%\begin{center}
%\begin{tabular}{ll}
%\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
%\\ \hline \\
%Dendrite         &Input terminal \\
%Axon             &Output terminal \\
%Soma             &Cell body (contains cell nucleus) \\
%\end{tabular}
%\end{center}
%\end{table}

%\section{Preliminaries}
%
%Consider a linear generative model for images: $ I = \phi \, a + \nu $, with $I \in \RR^{l \times n}$, $\phi \in \RR^{l \times m}$, and $\nu \in \RR^{l \times n}$. Each column of $I$ is a vector of discretely sampled pixels from an image patch, each column of $\phi$ is a basis vector, each column of $a$ is a vector of coefficients, and $\nu$ is i.i.d. Gaussian noise used to account for small variations in the pixels not well described by the model. In sparse coding the $a_{iu}$ are independent random variables with $P(a_{iu}) \propto \exp \{ -S(a_{iu}) \}$ and $S(\cdot)$ chosen to give $P(a_{iu})$ a peak at zero and heavy tails -- for example, $S(x) = |x|$. In this case, the $a$ and $\phi$ that maximize the posterior are found by the solution to $\arg \min_{a, \phi} || I - \phi \, a ||^2_F + \lambda || a ||_1$ where $\lambda$ is a weighting term that trades off sparsity in the $a$ solution for image reconstruction quality and $||\cdot||_F$ denotes the Frobenius norm. To avoid the trivial solution where the $\phi$ grow without bound we impose a uniform prior over basis functions with L2 norm less than 1.
%
%Solving this joint minimization is computationally infeasible, so instead of maximizing the posterior directly, we use an E-M algorithm to iteratively maximize a lower bound on the posterior.  In the E-step we compute
%\begin{equation}
%a^{(t)} = \arg \min_a || I - \phi^{(t)} \, a ||^2_F + \lambda || a ||_1
%\end{equation}
%and in the M-step we compute
%\begin{eqnarray*}
%\phi^{(t+1)} = \arg \min_\phi & &  || I - \phi \, a^{(t)} ||^2_F \\
% \mbox{s. t.}                 & &  \sum_{x} | \phi_{xi} |^2 \le 1 \, \forall i .
%\end{eqnarray*}
%For natural scenes, \cite{olshausen96emergence} showed that iterating a slight variation of this algorithm to convergence produces oriented, localized Gabors -- the same has been shown for this algorithm \cite{lee07}.  Note that by substituting an an i.i.d. Gaussian prior on the weights in each basis function $P(\phi_{xi}) \propto {\cal N}(0,1/\sqrt{2 \pi} \gamma)$ we obtain another algorithm that produces similar properties upon convergence with an M-step that is an unconstrained optimization problem:
%\begin{equation*}
%\phi^{(t+1)} = \arg \min_\phi || I - \phi \, a^{(t)} ||^2_F +
%                       \gamma || \phi ||^2_F .
%\end{equation*}
%For practical reasons it is more efficient to solve this M-step than the constrained M-step when the derivatives of the dual problem become unwieldy (as is the case in the feature transformation model described below).



==> content.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{What is {\em Thesis in a Box}?}

{\em Thesis in a Box} is a \LaTeX{} framework for formatting a PDF
doctoral dissertation at the University of California,
Berkeley.\footnote{I hope it will be useful to students filing at
  other schools, but the format may need to be changed to satisfy
  other school's requirements.}

\section{Why use PDF instead of PostScript?}

PDF has several advantages over PostScript: in many cases it is more
compact; more people have PDF readers than PostScript readers; and,
PDF readers have more functionality like hyperlinking and annotation.

{\em Thesis in a Box} uses the
\href{http://www.tug.org/applications/hyperref}{{\tt hyperref}}
package and compiles your \LaTeX{} source directly to PDF.  This gives
your thesis several nice features, which are described below.

\subsection{Bookmarks}

The first advantage is that, using Adobe Acrobat, the readers of your
thesis can quickly navigate the chapters and sections of your thesis
using the bookmark window.  If you are viewing this document in Adobe
Acrobat, look on the left hand side and you will see that you can
quickly navigate through this document.

\subsection{Hyperlinking}

The second advantage is that the following types of references are
automatically hyperlinked:
\begin{itemize}

  \item chapter and section references, including those in the table
  of contents (e.g., go to Chapter \ref{chap:files})

  \item equation references (e.g., check out \eqref{eq:example})

  \item citations (e.g., this document is \cite{TIAB2003})

  \item index references (e.g., this boldface \index{item}{{\bf item}}
  is indexed as ``item''---check the index at the back)

\end{itemize}

\subsection{Annotation}

PDF files support reader annotation, which can a useful way for your
thesis committee to comment on drafts.  

\subsection{Graphics}

Because your thesis is compiled directly to PDF, all graphics you
include must be in PDF format.  Thesis in a Box includes the package
\href{http://www.tug.org/tex-archive/help/Catalogue/entries/graphicx.html}{\tt
  graphicx}, so you can use the {\tt $\backslash$includegraphics}
command to include PDF graphics directly into your thesis.  If you
have used EPS graphics in the past, they can be converted to PDF
format using the Unix utility {\tt epstopdf}.  An example is given in
Figure \ref{fig:mote}.

\begin{figure}
\centering
\includegraphics[height=0.2\textheight]{mote.pdf}
\caption{A figure.  This caption is typeset in sans serif font to
  distinguish it from body text; you can turn this off if you like.}
\label{fig:mote}
\end{figure}

\section{Contributions}

{\em Thesis in a Box} is useful for a number of reasons.  First, it
implements the strict formatting requirements of the University of
California, Berkeley.  Second, it gives you easy examples of how to do
things in \LaTeX{} that you might not have done before, like citations,
indexing, tables of contents, etc.  Finally, {\em Thesis in a Box} comes
with a {\tt Makefile} which makes it really easy to compile your thesis.

\section{Outline of this thesis}

The rest of this document is structured as follows:
\begin{itemize}

  \item In Chapter \ref{chap:files} we describe the files in the
  distribution, and what you should (and should not) change to write
  your thesis.

  \item In Chapter \ref{chap:compile} we describe how to compile the
  \LaTeX{} thesis into PDF.  For a quick start, you can compile this
  document by typing {\tt make}.

\end{itemize}

\begin{subappendices}

\section{How to make an appendix}

Using the {\tt appendix} package, you can place appendices at the end
of chapters rather than at the end of the thesis.  This can make your
chapters more self-contained.

\end{subappendices}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Files}
\label{chap:files}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{\em Thesis in a Box} consists of a set of files, some of which you
will change, and others which you will not.  You will change the
following files:
\begin{itemize}

  \item {\tt frontmatter.sty}, which customizes the information in the
  front matter (e.g., thesis title, your name, etc.)

  \item {\tt abstract.tex}, the \LaTeX{} source of your abstract

  \item {\tt acknowledgements.tex}, the \LaTeX{} source of your
  acknowledgements

  \item {\tt commands.tex}, the \LaTeX{} source of all the extra
  commands you want included in the document, like package includes
  and command definitions

  \item {\tt content.tex}, the \LaTeX{} source of your thesis

  \item {\tt thesis.bib}, the Bib\TeX{} file containing your
  bibliography information

\end{itemize}
Do not change the following files, unless you know what you're doing:
\begin{itemize}

  \item {\tt thesis.tex}, the \LaTeX{} file that collects together
  several \LaTeX{} files to form your complete thesis

  \item {\tt frontmatter.tex}, the \LaTeX{} source of the front
  matter, including the title page, table of contents, etc.

  \item {\tt hyperref.cfg}, which customizes the PDF translation

  \item {\tt named.sty} and {\tt named.bst}, which implement the
  ``named'' Bib\TeX{} style

  \item {\tt Makefile}, which allows you to compile your thesis easily
  using {\tt make}

\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Compiling your thesis}
\label{chap:compile}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The {\tt Makefile} distributed with {\em Thesis in a Box} has been
designed to perform the following functions if and when they are
needed:
\begin{itemize}

  \item Compiling the sources using {\tt pdflatex}

  \item Creating the bibliography using {\tt bibtex}

  \item Creating the index using {\tt makeindex}

\end{itemize}
It is also sensitive to when \LaTeX{} must be run multiple times to
resolve cross-references.  There are two commands that are useful:
\begin{enumerate}

  \item {\tt make}: this performs all of the tasks above, resulting in
  the PDF file

  \item {\tt make clean}: this removes the PDF file as well as any
    intermediate files made by the {\tt make} process.  It does {\em
      not} remove other files like E-macs {\tt \~{}} files.

\end{enumerate}

To view your thesis, you can use Acrobat Reader or another PDF viewer
such as Apple Preview.  While you are writing your thesis, I recommend
using {\tt xpdf} as a viewer, because you can quickly reload the PDF
file to reflect editing changes by simply typing {\tt r}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Conclusion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Contributions of this thesis}

Okay, so {\em Thesis in a Box} is not as impressive as Einstein's
famous relation between matter and energy:
\begin{eqnarray}
E = mc^2 \label{eq:example}
\end{eqnarray}
But I hope it saves you some time.

\section{Directions for future research}

If anyone sees a nice way to improve {\em Thesis in a Box}, please let
me know (or better yet, do it and send me the result).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> dedication.tex <==
\vspace*{0.4\textheight}

\emph{Dedicated to ...}



==> fig_MPF/references.tex <==
\subsubsection*{References}

\small{


[1] Shlens et al. The Structure of Large-Scale Synchronized Firing in Primate Retina. Journal of Neuroscience (2009) vol. 29 (15) pp. 5022-5031

[2] Hyvarinen. Connections between score matching, contrastive divergence, and pseudolikelihood for continuous- É. IEEE Transactions on Neural Networks (2007)

[3] Broderick et al. Faster solutions of the inverse pairwise Ising problem. E-print arXiv (2007)

[4] Hinton et al. A fast learning algorithm for deep belief nets. Neural Comput (2006) vol. 18 (7) pp. 1527-1554

[5] Yuille. The Convergence of Contrastive Divergences. Collection (2005) pp. 1593-1600

[6] Hyvarinen. Estimation of non-normalized statistical models using score matching. Journal of Machine Learning Research (2005) vol. 6 pp. 695-709

[7] Carreira-Perpinan and Hinton. On contrastive divergence (CD) learning. Technical report, Dept. of Computere Science, University of Toronto (2004)

[8] Amit and Tsodyks. Image Analysis, Random Fields and Markov Chain Monte Carlo Methods. ($2^nd$ ed.). Book (2002)

[9] Li. Markov random field modeling in image analysis. Book (2002)

[10] Movellan et al. A Monte-Carlo EM approach for partially obserevable diffusion processes: Theory and applications to neural networks. Neural Computation (2002) vol. 14 (7) pp. 1507-1544

[11] Hinton. Training products of experts by minimizing contrastive divergence. Neural Computation (2002) vol. 14 (8) pp. 1771-1800

[12] Tanaka. Mean-field theory of boltzmann machine learning. Neural Comput Phys Rev E (1998)

[13] Kappen and Rodr?guez. Mean field approach to learning in Boltzmann Machines. Pattern Recognition Letters (1997)

[14] Jaakkola and Jordan. A variational approach to Bayesian logistic regression models and their extensions. Proceedings of the sixth international workshop on É (1997)

[15] Gilks et al. Markov Chain Monte Carlo in practice. Book (1996)

[16] Agmon-Snir and Segev. Signal delay and input synchronization in passive dendritic structures. J. Neurophysiol. (1993) vol. 70 pp. 2066-2085

[17] Movellan and McClelland. Learning continuous probability distributions with symmetric diffusion networks. Cognitive science (1993) vol. 17 pp. 463-496

[18] Ackley et al. A learning algorithm for Boltzmann machines. Cognitive science (1985) vol. 9 (2) pp. 147-169

[19] Pathria. [BOOK]ÊStatistical mechanics;(International series of monographs in natural philosophy, v. 45) tural É
. Pergamon (1972)

[20] Neal. Probabilistic inference methods using Markov chain Monte Carlo methods. citeseer.ist.psu.edu













Hyvarinen. Technical Report: http://www.cs.helsinki.fi/u/ahyvarin/papers/unsuper.shtml (2006)

Yuille. The Convergence of Contrastive Divergences. Collection (2005) pp. 1593-1600

Hyvarinen. Estimation of non-normalized statistical models using score matching. Journal of Machine Learning Research (2005) vol. 6 pp. 695-709

Carreira-Perpinan and Hinton. On contrastive divergence (CD) learning. Technical report, Dept. of Computere Science, University of Toronto (2004)

Amit and Tsodyks. Image Analysis, Random Fields and Markov Chain Monte Carlo Methods. ($2^nd$ ed.). Book (2002)

Li. Markov random field modeling in image analysis. Book (2002)

Hinton. Training products of experts by minimizing contrastive divergence. Neural Computation (2002) vol. 14 (8) pp. 1771-1800

Movellan et al. A Monte-Carlo EM approach for partially obserevable diffusion processes: Theory and applications to neural networks. Neural Computation (2002) vol. 14 (7) pp. 1507-1544

Gilks et al. Markov Chain Monte Carlo in practice. Book (1996)

Neal. Technical Report CRG-TR-93-1, Dept. of Computer Science, University of Toronto, ftp://ftp.cs.toronto.edu/pub/radford/review.ps.Z. (1993)

Agmon-Snir and Segev. Signal delay and input synchronization in passive dendritic structures. J. Neurophysiol. (1993) vol. 70 pp. 2066-2085

Movellan and McClelland. Learning continuous probability distributions with symmetric diffusion networks. Cognitive science (1993) vol. 17 pp. 463-496

Ackley et al. A learning algorithm for Boltzmann machines. Cognitive science (1985) vol. 9 (2) pp. 147-169



[] mean field theory and expansions

[] variational bayes techniques

[] other sampling or num. int. based methods

[] CD Hinton

[] Hyvarinen SM

[] Movellan Preprint

[] Jascha unpublished work

[] stat mech book

[] blog with materials

[] broderick et al inverse ising paper

[] Tka\v cik et al 2008

[] personal communication with jon shlens

[] jon shlens 2009 paper

[] DBN ref

[] RBM ref

[] MNIST postal data
}

@article{Ackley85,
AUTHOR = "Ackley, D. H. and Hinton, G. E. and Jejnowski, T. J.",
TITLE = "A learning algorithm for Boltzmann machines.",
JOURNAL = "Cognitive Science",
VOLUME = "9",
NUMBER = "2",
YEAR = "1985",
PAGES = "147-169"
}

@article{Hinton02,
AUTHOR = "Hinton, G. E.",
TITLE = "Training products of experts by minimizing contrastive divergence",
YEAR = "2002",
JOURNAL = "Neural Computation",
VOLUME = "14",
NUMBER = "8",
PAGES = "1771-1800"
}

@article{Hinton02,
AUTHOR = "Carreira-Perpinan, M. A. and Hinton, G. E.",
TITLE = "On contrastive divergence (CD) learning",
YEAR = "2004",
JOURNAL = "Technical report, Dept. of Computere Science, University of Toronto",
%VOLUME = "????",
%PAGES = "????"
}

@book{WINKLER02,
AUTHOR = "Amit, D.J. and Tsodyks, M.V.",
TITLE = "Image Analysis, Random Fields and Markov Chain Monte Carlo Methods.  ($2^{nd}$ ed.)",
YEAR = "2002",
PUBLISHER = "Springer-Verlag"
}

@article{Hyvarinen05,
AUTHOR = "Hyvarinen, A.",
TITLE = "Estimation of non-normalized statistical models using score matching.",
JOURNAL = "Journal of machine learning research",
VOLUME = "6",
PAGES = "695-709",
YEAR = "2005"
}

@article{Hyvarinen06,
AUTHOR = "Hyvarinen, A.",
TILE = "Connections between score matching, contrastive divergence, and pseudolikelihood for continuous-valued variables.",
JOURNAL = "Technical Report: http://www.cs.helsinki.fi/u/ahyvarin/papers/unsuper.shtml",
YEAR = "2006"
}

@article{Movellan93,
AUTHOR = "Movellan, J. R. and McClelland, J. L.",
YEAR = "1993",
TITLE = "Learning continuous probability distributions with symmetric diffusion networks",
JOURNAL = "Cognitive Science",
VOLUME = "17",
PAGES = "463-496"
}

@article{Movellan02,
AUTHOR = "Movellan, J. R. and Mineiro, P. and Williams, R. J.",
TITLE = "A Monte-Carlo EM approach for partially obserevable diffusion processes: Theory and applications to neural networks.",
JOURNAL = "Neural Computation",
VOLUME = "14",
NUMBER = "7",
PAGES = "1507-1544",
YEAR = "2002"
}

@book{Gilks96,
EDITOR = "Gilks, W. and Richardson, S. and Spiegelhalter, D. J.",
TITLE = "Markov Chain Monte Carlo in practice.",
PUBLISHER = "Chapman & Hall",
YEAR = "1996"
}

@book{Li01,
AUTHOR = "Li, S. Z.",
TITLE = "Markov random field modeling in image analysis.",
PUBLISHER = "Springer-Verlag",
YEAR = "2002"
}

@article{Neal93,
AUTHOR = "Neal, R. M.",
JOURNAL = "Technical Report CRG-TR-93-1, Dept. of Computer Science, University of Toronto, ftp://ftp.cs.toronto.edu/pub/radford/review.ps.Z.",
YEAR = "1993"
}

@incollection{Yuille04,
 author = {Alan {Yuille}},
 title = {The Convergence of Contrastive Divergences},
 booktitle = {Advances in Neural Information Processing Systems 17},
 editor = {Lawrence K. Saul and Yair Weiss and {L\'{e}on} Bottou},
 publisher = {MIT Press},
 address = {Cambridge, MA},
 pages = {1593-1600},
 year = {2005},
 original = "1593_268.PDF",
}

@article{WINKLER02,
AUTHOR = "Agmon-Snir, H. and Segev, I.",
TITLE = "Signal delay and input synchronization in passive dendritic
structures",
YEAR = "1993",
JOURNAL = "J. Neurophysiol.",
VOLUME = "70",
PAGES = "2066-2085"
}


